Finite sample inference for empirical Bayesian methods

In recent years, empirical Bayesian (EB) inference has become an attractive approach for estimation in parametric models arising in a variety of real-life problems, especially in complex and high-dimensional scientific applications. However, compared to the relative abundance of available general methods for computing point estimators in the EB framework, the construction of confidence sets and hypothesis tests with good theoretical properties remains difficult and problem specific. Motivated by the universal inference framework of Wasserman et al. (2020), we propose a general and universal method, based on holdout likelihood ratios, and utilizing the hierarchical structure of the specified Bayesian model for constructing confidence sets and hypothesis tests that are finite sample valid. We illustrate our method through a range of numerical studies and real data applications, which demonstrate that the approach is able to generate useful and meaningful inferential statements in the relevant contexts.

==> Table4FSEBnew.tex <==
% latex table generated in R 4.1.0 by xtable 1.8-4 package
\begin{table}
\caption{\label{tab:beta-binomial sim - test}Experimental results
for testing the hypothesis $\text{H}_{0}$: $\theta_{i1}^{*}=\theta_{i2}^{*}$
for Beta--binomial count series models. The Rejection proportion columns
report the average number of rejections, from 100 test replicates, at levels
of significance $\alpha\in\left\{ 0.05,0.005,0.0005\right\} $.}

\centering{}
\begin{tabular}{lcllll}
  \hline
   &   &   & \multicolumn{3}{c}{Rejection proportion at level $\alpha$} \\
$n$ & $\bm{\psi}$ &$\Delta$ & $0.0005$ & $0.005$ & $0.05$  \\ 
  \hline
  \hline 
  10 & $(2,2)$&    0 &                           0.000 & 0.000 & 0.000 \\ 
                  & & 0.2 &                      0.001 & 0.003 & 0.021 \\ 
                  & & 0.5 &                      0.279 & 0.475 & 0.718 \\ 
                  & & 0.9 &                      1.000 & 1.000 & 1.000 \\ 
       &$(2,5)$ &    0 &                         0.000 & 0.000 & 0.000 \\ 
                  & & 0.2 &                      0.000 & 0.001 & 0.022 \\ 
                  & & 0.5 &                      0.266 & 0.462 & 0.695 \\ 
                  & & 0.9 &                      0.991 & 1.000 & 1.000 \\ 
       &$(5,2)$ &    0 &                         0.000 & 0.000 & 0.000 \\ 
                  & & 0.2 &                      0.000 & 0.002 & 0.035 \\ 
                  & & 0.5 &                      0.279 & 0.465 & 0.709 \\ 
                  & & 0.9 &                      1.000 & 1.000 & 1.000 \\ 
\hline 
100 &$(2,2)$ &    0 &                     0.000 & 0.000 & 0.000 \\
                  & & 0.2 &               0.000 & 0.003 & 0.034 \\
                  & & 0.5 &               0.281 & 0.478 & 0.704 \\
                  & & 0.9 &               0.993 & 0.997 & 1.000 \\
       &$(2,5)$    & 0 &                  0.000 & 0.000 & 0.000 \\
                  & & 0.2 &               0.000 & 0.002 & 0.027 \\
                  & & 0.5 &               0.283 & 0.474 & 0.710 \\
                  & & 0.9 &               0.990 & 0.995 & 0.998 \\
       &$(5,2)$ &    0 &                  0.000 & 0.000 & 0.000 \\
                  & & 0.2 &               0.000 & 0.004 & 0.045 \\
                  & & 0.5 &               0.275 & 0.469 & 0.703 \\
                  & & 0.9 &               0.987 & 0.997 & 1.000 \\
  \hline 
1000 &$(2,2)$ &    0 &             0.000 & 0.000 & 0.000 \\
                    & & 0.2 &      0.000 & 0.003 & 0.029 \\
                    & & 0.5 &      0.268 & 0.463 & 0.696 \\
                    & & 0.9 &      0.987 & 0.997 & 1.000 \\
         &$(2,5)$ &    0 &         0.000 & 0.000 & 0.000 \\
                   & &  0.2 &      0.000 & 0.003 & 0.027 \\
                   & &  0.5 &      0.268 & 0.465 & 0.698 \\
                   & &  0.9 &      0.987 & 0.996 & 1.000 \\
        &$(5,2)$ &     0 &         0.000 & 0.000 & 0.000 \\
                   & &  0.2 &      0.000 & 0.005 & 0.047 \\
                   & &  0.5 &      0.270 & 0.465 & 0.699 \\
                   & &  0.9 &      0.990 & 0.997 & 1.000 \\
   \hline
\end{tabular}
\end{table}

